Neural-Symbolic Logic Query Answering in Non-Euclidean Space

Answering complex first-order logic (FOL) queries on knowledge graphs is essential for reasoning. Symbolic methods offer interpretability but struggle with incomplete graphs, while neural approaches generalize better but lack transparency. Neural-symbolic models aim to integrate both strengths but often fail to capture the hierarchical structure of logical queries, limiting their effectiveness. We propose HYQNET, a neural-symbolic model for logic query reasoning that fully leverages hyperbolic space. HYQNET decomposes FOL queries into relation projections and logical operations over fuzzy sets, enhancing interpretability. To address missing links, it employs a hyperbolic GNN-based approach for knowledge graph completion in hyperbolic space, effectively embedding the recursive query tree while preserving structural dependencies. By utilizing hyperbolic representations, HYQNET captures the hierarchical nature of logical projection reasoning more effectively than Euclidean-based approaches. Experiments on three benchmark datasets demonstrate that HYQNET achieves strong performance, highlighting the advantages of reasoning in hyperbolic space.

==> 006other.tex <==

\begin{figure*}
	\centering
	\includegraphics[width=0.8\textwidth]{pics/llm.png}
	\vspace{-1\baselineskip}
	\caption{Three ways to combine LLMs with knowledge graph reasoning.}
	\label{llm}
\end{figure*}


with the advent of ChatGPT, large language models have demonstrated great performance in many downstream tasks. Previously, we introduced knowledge graph reasoning. We know that knowledge graphs contain accurate structural knowledge and are very interpretable, however, most knowledge graphs are incomplete, lack language understanding. While language models are general knowledge, they are good at language understanding. However, they suffer from hallucination, lack interpretation, lacking new knowledge. By combining them together, we can build a model that is not only accurate but also interpretable. 

When combining knowledge graphs with large language models, there are three different ways. The first category is letting LLMs enhance knowledge graph reasoning, where LLMs serve as a component in the reasoning process. The second category is Knowledge graph reasoning enhance LLMs where knowledge graph reasoning can be used to mitigate the LLM’s hallucination problem. Finally, integrating knowledge graph reasoning with LLMs in a mutually beneficial way, so that they can help each other. Figure ~\ref{llm} shows the classification. 


\subsubsection{Knowledge graph enhances LLMs.}  Many methods have been proposed to utilize knowledge graph to boost the LLMs performance. In QA-GNN ~\cite{qagnn}, it combines LLM and knowledge graph to answer multi-choice questions. First of all, given a QA context, it will use the language model to encode question to a vector presentation, then use stand method to retrieve a knowledge graph subset, like linking entities and get their neighbors, and reasoning according to the subgraph. 
Then QA-GNN is based on two core ideas. First, in order to better identify which knowledge graph nodes relevant to current question, they propose language condition KG nodes scoring where they use a pretrained language model to compute the probability of each entity condition on the current question. 
Secondly, to jointly reason with language models, they connect the question text and kg to form a joint graph, which we call working graph, they mutually update their representations, through graph neural networks. Finally, they combine the representation of the language model and kg to predict the final answer. 
Following this direction, GreaseLM ~\cite{greaselm} merges LM with graph neural network by using a merging layer. To encode the knowledge graph structure information, multiple merging layers are used.

Now, we have introduced how to use knowledge graphs to help retrain language models to better answer different types of questions. However, when the size of the model becomes large, retrain or finetune the model will be very time consuming. An alternative way is to retrieval knowledge from external sources to help the language model generate correct answers. This approach allows for more targeted adjustments without the need for extensive retraining. This type of method is called Retrieval-Augmented Generation short for RAG. 

In KG-GPT ~\cite{kim2023kg}, the authors propose a method to utilize language models and knowledge graphs to answer more complex natural language questions. The idea is that a sentence of question, it uses llms to decompose the original sentence to several sub-sentences and find answers for each sub-sentence. And finally, find the answer for the whole sentence.
In REPLUG ~\cite{replug}, a new retrieval-augmented LM framework where the language model is viewed as a black box and the retrieval component is added as a tunable plug-and-play module. Given an input context, REPLUG first retrieves relevant documents from an external corpus. The retrieved documents are prepended to the input context and fed into the black-box LM to make the final prediction. Because the LM context length limits the number of documents that can be prepended, they also introduce a new ensemble scheme that encodes the retrieved documents in parallel with the same black-box LM. Then we pass the concatenation of each retrieved document with the input context through the LM in parallel, and ensemble the predicted probabilities. 
They have also developed REPLUG LSR. Instead of adjusting the language model to fit the retriever, they adapt the retriever to the language model. they train it to find documents that help improve the language model's understanding, while keeping the language model unchanged. The training process involves four steps: (1) finding and assessing the relevance of documents, (2) scoring these documents using the language model, (3) adjusting the retrieval model based on how different the retrieval and language model scores are, and (4) updating the index of the data in real-time.

Previous approaches of retrieval-augmented language models can only answer questions where answers are contained locally within regions of text and fail on answering global questions such as “what are the main themes in the dataset?” To solve these questions, the work proposes a method called GraphRAG ~\cite{edge2024local} which is a two-step process. The approach uses an LLM to build a graph-based text index in two stages: first to derive an entity knowledge graph from the source documents, then to pregenerate community summaries for all groups of closely-related entities. Given a question, each community summary is used to generate a partial response, before all partial responses are again summarized in a final response to the user. 



\subsubsection{LLMs enhances knowledge graph reasoning.} Traditional methods retrieve information from KGs, augment the prompt accordingly, and feed the increased prompt into LLMs. In this paradigm, LLM plays the role of translator which transfers input questions to machine-understandable command for KG searching and reasoning, but it does not participate in the graph reasoning process directly. Its success depends heavily on the completeness and high quality of KG, which means that if the knowledge graph contains many missing edges, the answer won’t be good. So, recently, some people tried to explore how to mitigate the knowledge graph incompleteness problem by treating the LLM as an agent to travel KGs and perform reasoning based on paths. In Think-on-Graph ~\cite{sun2023think}, LLM is treated as an agent to traverse on knowledge graph to find answers. Now, let’s see an example, given question “What is the majority party now in the country where Canberra is located?” The llm identitied the topic entity is Canberra, by checking its local neighbourhood, Australia has the highest score. But the LLM notices that there is not enough information to get the answer. So it travels to Australia and check its neighbors. 

\subsubsection{LLMs and knowledge graph reasoning mutually help each other.}  Finally, let us introduce the third part, how to let knowledge graph reasoning and large language models mutually help each other. 

One of the most important tasks in knowledge graph reasoning is to learn the embedding for the KG entities. It has been shown that the learned embedding from KG can be used to improve the performance of Pre-trained Language Models. On the other hand, for each node in the knowledge graph, we can find many text descriptions to describe it. This text information can be used to learn the node embedding. The strong ability of pre-trained language model can help us learn the embedding. So, in KEPLER ~\cite{kepler}, they propose a model which can also solve two problems at the same time. 
In this paper, Roberta is chosen as the encoder. Given a triplet, each node has a text description. Roberta is used to learn entity embedding. And the learned embedding will be used to calculate the knowledge graph embedding loss. On the other hand, conventional masked language model is used. It requires the model to predict the masked token within the text. The final loss is the summation of these two losses. 

 
To leverage the structure information during the reasoning process, In ~\cite{jaket}, this work proposes to use a graph attention network to provide structure-aware entity embeddings for language modeling. More specifically, the language module produces contextual representations as initial embeddings for KG entities and relations given their descriptive text. Then, graph neural network is used to update the node embedding and relation embedding. 
Next, the learned knowledge graph embedding will be used as the input of the language model. And the output of the language model will be used to solve different downstream tasks.  There are several advantages of this method. For example, the joint pre-training effectively projects entities/relations and text into a shared semantic latent space, which eases the semantic matching between them. 




==> 007llm.tex <==


With the advent LLMs, it shows good performance in many applications. However, LLMs suffer from hallucination problem. While Knowledge graph contains the factual knowledge and also the structure information. Recently, there is a new trend to combine LLMs with knowledge graph reasoning.
In this section, we describe combining large language models with knowledge graph reasoning from the following three categories: how LLMs can facilate knowledge graph reasoning, how knowledge graph reasoning to faciliate large language models and how they can mutually benefit each other. 

Essentially, a language model is a probability distribution over strings of text. The language model essentially functions as a black box that assigns probability numbers to different strings. These probabilities reflect how frequently you expect to encounter that string. For example, if we have four different strings, a language model would assign probabilities to those strings. A good string will have high probability, whereas a bad string will have low probability. Here the second string, being not good, will have low probabilities. Now, with the advent of ChatGPT, large language models have demonstrated great performance in many downstream tasks. These large, general-purpose language models can be pre-trained and then fine-tuned for specific purposes. Examples include GPT-3.5, GPT-4, Llama2, and Llama3. 

In recent years, large language models keep getting bigger, going from 0.1 billion to a massive 500 billion parameters. This growth isn't just about big numbers; it means they work better. As they get larger, these models get better at understanding and creating language, making them more accurate and efficient at handling tough tasks.

Here, we give some large language models which have been released in recent years. In 2023, LLama2 and GPT-4 were two major milestones in the development of large language models. LLama2 is an opensource language model which can achieve a similar performance as ChatGPT in many NLP tasks and inspires new models. Meanwhile, GPT-4 set new records in size and performance. This timeline illustrates the rapid progression and improvement of large language models in just a few short years.

Previously, we introduced knowledge graph reasoning. We know that knowledge graphs contain accurate structural knowledge and are very interpretable, however, most knowledge graphs are incomplete, lack language understanding. While language models are general knowledge, they are good at language understanding. However, they suffer from hallucination, lack interpretation, lacking new knowledge. By combining them together, we can build a model that is not only accurate but also interpretable. 

When combining knowledge graphs with large language models, there are three different ways. The first category is letting LLMs enhance knowledge graph reasoning, where LLMs serve as a component in the reasoning process. The second category is Knowledge graph reasoning enhance LLMs where knowledge graph reasoning can be used to mitigate the LLM’s hallucination problem. Finally, integrating knowledge graph reasoning with LLMs in a mutually beneficial way, so that they can help each other. 

\subsection{Knowledge graph enhance LLMs}

Now, let’s first see the first category. LLMs enhance knowledge graph reasoning. 

Given a commonsense question. “If it is not used for hair, a round brush is an example of what?” along with some answer choices. The goal of this paper is to correctly answer the multi-choice questions by utilizing LLMs and KGs. Question answering is a fundamental problem in natural language processing. To do well, the system needs to access a lot of knowledge and reason about it. Typically, knowledge can be encoded in large language models, or represented in structured knowledge graphs, where entities are represented as nodes and relations are represented as edges. 

Pretrained language models have shown great performance in many QA tasks. But at the same time, they may not work well for logical reasoning. On the other hand, KGs are more explicitly represented, and contain structure reasoning. But the knowledge graph is incomplete and noisy. Thus, in order to leverage both sources of knowledge to enhance question answering performance, there are two challenges: how to identify the relevant information in the knowledge graph, and how to jointly reason over the text and the knowledge graph.

In this work, the authors present QA-GNN, a hybrid model, which combines LLM and knowledge graph to solve this problem. Here is the overview of QA-GNN. First of all, given a QA context, it will use the language model to encode question to a vector presentation, then use stand method to retrieve a knowledge graph subset, like linking entities and get their neighbors, and reasoning according to the subgraph. 

Then QA-GNN is based on two core ideas. First, in order to better identify which knowledge graph nodes relevant to current question, they propose language condition KG nodes scoring where they use a pretrained language model to compute the probability of each entity condition on the current question. 

Secondly, to jointly reason with language models, they connect the question text and kg to form a joint graph, which we call working graph, they mutually update their representations, through graph neural networks. Finally, they combine the representation of the language model and kg to predict the final answer. 

To learn the knowledge graph information, they design attention-based graph neural network. The basic idea of gnn is to update the presentation of each node by letting neighboring nodes send messages to each other for multiple layers. Concretely, they update the representation of each node t according to the formulations in the left hand of this slide.

In the experiment, two benchmarks were used. One is commonsense QA, which has multiple choice questions. Another dataset is openbookQA, which has multiple choice questions. We can find that QA-GNN achieves improved performance over previous systems on all the QA benchmarks. 

\subsubsection{Retrieval augmented generation}
Now, we have introduced how to use knowledge graphs to help retrain language models to better answer different types of questions. However, when the size of the model becomes large, retrain or finetune the model will be very time consuming. An alternative way is to retrieval knowledge from external sources to help the language model generate correct answers. This approach allows for more targeted adjustments without the need for extensive retraining. This type of method is called Retrieval-Augmented Generation short for RAG. 

Let’s see a simple example. In this paper, the authors propose a method to utilize language models and knowledge graphs to answer more complex natural language questions. The idea is that a sentence of question, it uses llms to decompose the original sentence to several sub-sentences and find answers for each sub-sentence. And finally, find the answer for the whole sentence.
More specifically, KG-GPT consists of three steps: 1) Sentence (Claim / Question) Segmentation, 2) Graph Retrieval, and 3) Inference. During Sentence Segmentation, a sentence is partitioned into discrete sub-sentences, each aligned with a single triple (i.e. [head, relation, tail]). The subsequent step, namely Graph Retrieval, retrieves a potential pool of relations that could bridge the entities identified within the sub-sentences. Then, a candidate pool of evidence graphs (i.e. sub-KG) is obtained using the retrieved relations and the entity set. In the final step, the obtained graphs are used to derive a logical conclusion, such as validating a given claim or answering a given question.
For the experiment, we can find that it significantly outperforms large language models, like ChatGPT with more than 40\% in average. While it can achieve the comparable performance compared to the state-of-the-art embedding models EmbedKGQA when the knowledge graph is full. 

--

Previous approaches of retrieval-augmented language models require access to the internal LM representations, and are thus difficult to be applied to very large LMs. In addition, many best-in-class LLMs can only be accessed through APIs. Internal representations of such models are not exposed and fine-tuning is not supported.

In this work, we introduce REPLUG (Retrieve and Plug), a new retrieval-augmented LM framework where the language model is viewed as a black box and the retrieval component is added as a tunable plug-and-play module.

Given an input context, REPLUG first retrieves relevant documents from an external corpus. The retrieved documents are prepended to the input context and fed into the black-box LM to make the final prediction. Because the LM context length limits the number of documents that can be prepended, we also introduce a new ensemble scheme that encodes the retrieved documents in parallel with the same black-box LM, allowing us to easily trade compute for accuracy. Then we pass the concatenation of each retrieved document with the input context through the LM in parallel, and ensemble the predicted probabilities. 

We've also developed REPLUG LSR. Instead of adjusting the language model to fit the retriever, we adapt the retriever to the language model. We train it to find documents that help improve the language model's understanding, while keeping the language model unchanged. Our training process involves four steps: (1) finding and assessing the relevance of documents, (2) scoring these documents using the language model, (3) adjusting the retrieval model based on how different the retrieval and language model scores are, and (4) updating the index of the data in real-time.

--

Previous approaches of retrieval-augmented language models can only answer questions where answers are contained locally within regions of text and fail on answering global questions such as “what are the main themes in the dataset?”

To solve these questions, the work proposes a method called GraphRAG which is a two-step process. The approach uses an LLM to build a graph-based text index in two stages: first to derive an entity knowledge graph from the source documents, then to pregenerate community summaries for all groups of closely-related entities. Given a question, each community summary is used to generate a partial response, before all partial responses are again summarized in a final response to the user. 

In Baseline rag, what you do is you take a private data set, you chunk it up using embeddings, and you store it into a vector database. Then you perform your neighbor search, and you can use those nearest neighbor searches to augment the context window.

Graph rag is a parallel process to the way that Baseline rag works. we ask the LLM to perform reasoning operations over top of each sentence in a single pass through over all of the data. We use LLMs to find all the entities and their relationship according to the text data, and create a knowledge graph. 
So, once we create these knowledge graphs, we can utilize graph machine learning to do divide the graph into different communities and generate summaries for each community at different levels. Finally, given a question, each community summary is used to generate a partial response before all partial responses are again summarized in a final response to the user.



\subsection{LLMs enhance knowledge graph reasoning}

Now, we have talked about how to use knowledge graphs to help large language models. In the next part, I will introduce how to use llms to help us better solve knowledge graph reasoning problems. 


Traditional methods retrieve information from KGs, augment the prompt accordingly, and feed the increased prompt into LLMs. In this paradigm, LLM plays the role of translator which transfers input questions to machine-understandable command for KG searching and reasoning, but it does not participate in the graph reasoning process directly. Its success depends heavily on the completeness and high quality of KG, which means that if the knowledge graph contains many missing edges, the answer won’t be good. So, recently, some people tried to explore how to mitigate the knowledge graph incompleteness problem by treating the LLM as an agent to travel KGs and perform reasoning based on paths. 

For example, given question “What is the major party now in the country where Canberra is located?”. Directly using LLM to answer the question will lead to some wrong answers. While existing LLMs plus KG methods will transform the natural language question to a symbolic SPARQL query and retrieve information from KGs, augment the prompt accordingly, and feed the increased prompt into LLMs. However, its success depends heavily on the completeness and high quality of KG. For example, although LLM successfully identified necessary relation types required to answer the question, the absence of the relation “majority party” leads to a failure in retrieving the correct answer.

In this work, LLM is treated as an agent to traverse on knowledge graph to find answers. Now, let’s see an example, given question “What is the majority party now in the country where Canberra is located?” The llm identitied the topic entity is Canberra, by checking its local neighbourhood, Australia has the highest score. But the LLM notices that there is not enough information to get the answer. So it travels to Australia and check its neighbors. Similarly, at this time, Anthony Albanese gets the highest score. By checking its neighbors, it can find the correct answer Labor Party. 


\subsection{Mutually benefit each other}

Finally, let us introduce the third part, how to let knowledge graph reasoning and large language models mutually help each other. 

One of the most important tasks in knowledge graph reasoning is to learn the embedding for the KG entities. Some commonly used methods include TransE, TransH or graph neural networks and so on. It has been shown that the learned embedding from KG can be used to improve the performance of Pre-trained Language Models. On the other hand, for each node in the knowledge graph, we can find many text descriptions to describe it. This text information can be used to learn the node embedding. The strong ability of pre-trained language model can help us learn the embedding. So, in this paper, they propose a model which can also solve two problems at the same time. 

In this paper, Roberta is chosen as the encoder. Given a triplet, each node has a text description. Roberta is used to learn entity embedding. And the learned embedding will be used to calculate the knowledge graph embedding loss. On the other hand, conventional masked language model is used. It requires the model to predict the masked token within the text. The final loss is the summation of these two losses. 

In the experiment, we can see that the proposed method can achieve the state of the art performance on knowledge graph completion task and also various NLP tasks. (two minutes)


When the entity has text description, we can use language model to learn its embedding. But the naïve transE based method may not have enough power to capture the structure information of the knowledge graph.  

To leverage the structure information during the reasoning process, this work proposes to use a graph attention network to provide structure-aware entity embeddings for language modeling. More specifically, the language module produces contextual representations as initial embeddings for KG entities and relations given their descriptive text. Then, graph neural network is used to update the node embedding and relation embedding. 

Next, the learned knowledge graph embedding will be used as the input of the language model. And the output of the language model will be used to solve different downstream tasks.  There are several advantages of this method. For example, the joint pre-training effectively projects entities/relations and text into a shared semantic latent space, which eases the semantic matching between them. 

In the experiment, we can find that the proposed method can achieve State of the art performance on KE task, and also State of the art performance on various NLP tasks






==> revision.tex <==

\section{Timeline}

\begin{itemize}
    \item Revise paper. Covid19 experiments. Dec 18 - Dec 25.
    \item Revise paper. Dec 25 - Dec 31.
\end{itemize}



==> theme/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering
